Learning migration models for supporting incremental language migrations of software applications

Context: A Legacy system can be defined as a system that significantly resists modification and evolution. According to the literature, there are two main strategies to migrate a legacy system: (a) to replace the legacy system by a new one, (b) to incrementally migrate parts from the legacy system to the new one. Incremental migration allows developers to better control the risks that may occur during the migration process. However, this strategy is more complex because it requires decomposition of the legacy system into different parts, e.g. a set of files, and to define the order of migration of them along the migration process. To our knowledge, there is no approach to support developers on those activities. Objective: This paper presents an approach, named MigrationExp, to support incremental language migrations of applications from one source language to another target language. MigrationExp recommends the files that should be migrated first in a particular migration iteration. As a novelty, our approach relies on a ranking model learned, using a learning-to-rank algorithm, from migrations made by developers. Method: We validate our approach in the context of the migrations of Android apps, from Java to Kotlin, a new official language for Android. We train our model using migrations of Java code to Kotlin written by developers on open-source applications. Results: The results show that, on the task of proposing files to migrate, our approach outperforms a previous migration strategy proposed by Google, in terms of its ability to accurately predict empirically observed migration orders. Conclusion: Since most Android applications are written in Java, we conclude that approaches to support developers such as MigrationExp may significantly impact the development of Android applications.

==> MigrationExpert (29)/oldtext.tex <==
%\todo{improve or remove}
%Let's give a simple example showed in Figure~\ref{cap6:fig:ranking_evaluation}  that illustrates how  our evaluation works.
%Given as input a project which in its last version (commit \#2) has 4 Java files ($A, C, D$ and $E$), since commit \#2  migrates one file ($A$), it becomes a query that contains one document per file.
%Then, our model generates a ranking of files containing all project files on that version (commit \#2), i.e., a ranking of documents composed of $A$, $C$, $D$ and $E$.
%This ranking is then analyzed based on the position of the \emph{relevant} documents (i.e., those from migrated files such as $A$) to compute the recommendation performance. 


%\todo{????}

%%%%%%% OLD intro



%% Kotlin + Announced
In 2017, Google promoted Kotlin, a programming language that combines functional and object-oriented features, as an official Android language.
More recently, in 2019, Google declared that Android became `Kotlin-first', which means that new API, libraries, documentation will target Kotlin and eventually Java~\cite{AndroidDevelopers2019}.
Since then, Google has advised developers to create new applications using Kotlin instead of Java~\cite{AndroidDevelopers2020b}.


Kotlin is compiled to Java byte-code, which means that 
it is interoperable with Java, i.e., Kotlin code can invoke code written in Java and vice-versa, both running on the same underlying JVM.
Thanks to this interoperability, developers of Java-based Android applications
can:
\begin{inparaenum}[i)]
\item add new Kotlin code and maintain the existing Java code, and/or
\item migrating some parts of theirs apps written in Java code to Kotlin.
\end{inparaenum}
Recent research has shown that the 19\% of Android applications completely migrated from Java to Koltin were \emph{gradually} migrated~\cite{GoisMateus2019}.


%%%%
Moreover, some popular commercial Android applications also gradually migrated from Java to Kotlin.
For instance, Duolingo, a free science-based language education platform~\cite{duolingo_website}, was migrated completely in 2 years. 
Figure~\ref{cap6:fig:duo} shows the evolution of the amount of Java and Kotlin code from Duolingo.
During that period, Java files were progressively migrated to Kotlin, i.e., a commit migrated a subset of Java files, leaving other files in Java.

The \emph{gradual} migration allows developers  
to:
\begin{inparaenum}[\it a)]
\item migrate a subset of Java files, 
\item exhaustively test the migrated code to verify that the migrated code preserves the expected behavior,
and 
\item commit (and eventually release) a new version of their app before continuing with the migration of other files. 
\end{inparaenum}
As Duolingo's developers report~\cite{duolingo_migration2020}, gradual migration allowed them to apply strict testing, code review and code style of each part of the application that was migrated.

Gradual migration faces several challenges.
This paper focuses on a particularly one:
given a version of the program to migrated (composed by not yet migrate and, eventually, some migrated code), a developer should select a set of files that she/he wants to migrate on that migration step.
This selection could be complex as:
\begin{inparaenum}[\it a)]
\item it could exist several candidate files to migrate, and 
\item the wrong selection of files to be migrated could increase the migration effort due to emerging errors~\cite{AbdelAziz2020MigEnterprise,Nizet2018StoryMigration} or additional modifications on files not affected on the migration step. 
\end{inparaenum}
Unfortunately, existing guidelines on migration give high-level pieces of advice or guidance. For instance, Google only suggests that the migration from Java to Kotlin on Android could start by migrating classes in the following order: class model first, then tests, utility functions, and, finally other classes~\cite{AndroidDevelopers2020a}.
%
However, it does not include any guidance for helping developers to decide, for instance, which subset of model classes could be more convenient to migrate first. 

In this paper, we present a novel approach, named \approach{}, that assists developers during the migration process by recommending a set of candidate Java files that could be migrated in the current migration step.

This work is novel: to our knowledge, no previous work has focused on recommendations of language migrations based on previous migrations done by developers.
This approach could complement other tools used by developers during migrations, for example, the automated Java-to-Kotlin file converter tool provided by IDEs such as Android Studio.


We build our approach applying the supervised machine learning technique \emph{learning-to-rank} to create a model that suggests the files to migrates.
The model is learned from real migrations from Java to Kotlin written by developers in open-source projects.
Our intuition is that using information from these migrations, our model captures the rationale behind these migrations.
We trained and evaluated our approach with commits that migrated Java code to Kotlin from \numprint{1457} open-source applications.
To the best of our knowledge, no work has proposed a machine learning-based approach in the context of Android application migration.


%\todo{R2: will there be a general standard, logic, or strategy of how should the migration implement? And how should it be? These should be the questions to be answered or studied first?}

%The result of this paper is: our approach outperforms the random approach by at least 38\%, considering the Mean Average Precision (MAP).\todo{update}
The results of this paper show that \approach{} obtains a mean average precision (MAP metric~\cite{baeza1999modern}) higher than a strategy that follows Google's guideline \cite{AndroidDevelopers2020a}.
We consider that the proposed approach is an initial step towards a fully automated recommendation system to support applications' migration.


The contributions of this paper are:
\begin{itemize}
    \item A benchmark of projects that performed migrations from Java to Kotlin.
    \item An approach that recommends migrations at file level from one programming language to another.
%    \item A static analyzer tool that identifies 12 metrics exclusive to Android applications.\footnote{https://anonymous.4open.science/r/fe5cf980-060b-49ad-81b5-28de22f26360/}\todo{Is this important?? }
\end{itemize}

The paper continues as follows.
Section \ref{sec:term} explains the terminology used along the paper.
Section \ref{sec:approach} characterizes our approach.
Section \ref{sec:methodology} outlines the methodology used to evaluate our approach.
Section \ref{sec:evaluation} reports the evaluation results.
Section \ref{cap6:sec:discussion} discusses the consequences of our results and future work.
Section \ref{sec:threatsvalidity} presents the threats to validity.
Section \ref{sec:relatedwork} presents the related work.
Section \ref{sec:conclusion} concludes the paper.
All the data presented in this paper is publicly available in our appendix: \url{https://anonymous.4open.science/r/fe5cf980-060b-49ad-81b5-28de22f26360}.


\begin{figure}[t]
    \centering
    \includegraphics[width=0.75\columnwidth]{duolingo_evolotion.png}
    \caption{Evolution of the number of lines (LOC, axis X) of Java and Kotlin along with the Duolingo application's migration process~\cite{duolingo_migration2020} since 2014 (Axis Y).}
    %Axis Y shows the amount of code (SLOC) written, and axis X the time from 2014.}
    \label{cap6:fig:duo}
\end{figure}  


%%%%%%%%% OLd Overview


\subsection{Overview}

\todo{for the moment, let's keep this overview here, it's quite specific to move to the new vision section.}

%Our intention is to capture real migrations  
We build our approach \approach{} using information from projects that have done file migrations from one programming language to another.
\todo{move to the concepts section}
Our intuition is that by analyzing those migrations, we can create a model that captures the rationale behind these migrations, i.e., the developers' experience on migrations.
Then we can use it to recommend files to be migrated.


Our approach consists of two phases as Figure~\ref{fig:app:overview} illustrates: 
\begin{inparaenum}[\it a)]
\item the development phase, and 
\item the serving phase. 
\end{inparaenum}
In the development phase, our approach learns a model from migrations from language $lang_1$ (e.g., Java) to $lang_2$ (e.g., Kotlin), done by developers on open-source projects.  
Then, in the serving phase, given a project $P$ as input, the model generated in the development phase is used to recommend file-level migrations: the model produces a list of candidate files to be migrated.
Now, we give a summary of both phases from our approach.

\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.85\textwidth]{methodology.png}
    \caption{We apply two phases: \emph{development}, where we learn a ranking model, and \emph{serving} phase, where we use the model in production.}
    \label{fig:app:overview}
\end{figure*} 

\subsubsection{Development phase}
\label{cap6:sec:design:approach:dev}


\approach{} is built using learning to rank, a supervised machine learning algorithm. Consequently, we need to provide example data to train our model.
Each example is described by a \emph{vector} of measurements or \emph{features} and a label that denotes the category or class the example belongs to~\cite{Hall1998}.
In our case, we use data from projects that have been migrated from one programming language to another to create \approach{}'s training set.
To this end, for each commit of these projects, we analyze their files to create a \emph{vector} of features that describe them by extracting a set of metrics and classifying them as migrated or not migrated (label).
These vectors are the training data used by our approach to learning a model.
Finally, once we trained our model, it is deployed, and it is ready to be used in the serving phase.


\subsubsection{Serving phase}
\label{sec:serving}

In the serving phase, our approach takes as input a program $P$, written partially or totally using $lang_1$, which developers aim to migrate to $lang_2$. 
As done in the development phase, our approach extracts features from the project's files, i.e., candidates files to migrate, and creates for each file one vector of features, as done during the development phase.
These vectors are given as input to our model.
Finally, using this information, the model learned in the development phase sorts the project's files according to their relevance and returns the list of recommended files to be migrated.


%Figure~\ref{cap6:fig:ranking_overview} shows an example of this phase. 
Let us show an simple example for describing this phase.
The approach takes as input a project composed of 5 files where 4 files ($A.lang_1$, $B.lang_1$, $C.lang_1$ and $E.lang_1$) could be migrated, and one $D.lang_2$ already migrated.
The learned rank model ranks the 4 files based on the experience of developers by migrating similar files (i.e., similar vector features). 
In this example, the developer could start migrating the files at the top of the recommendation, e.g., $E.lang_1$, then testing the migrated app, committing the changes, and generating a new version to publish. 
Those activities conform one step on the gradual migration process.
Note that in migrations that involve fully interoperable languages (e.g., Java and Kotlin) the migrated files (e.g., $D.lang_2$) could continue interacting with the not migrated (e.g., $B.lang_1$).

%To our knowledge, all existing guidelines on migration give high-level pieces of advice or guidance. 
%For instance, Google only suggests that the migration from Java to Kotlin on Android could start by migrating classes in the following order: class model first, then tests, utility functions, and, finally other classes~\cite{AndroidDevelopers2020a}.
%However, it does not include any guidance for helping developers to decide, for instance, which subset of model classes could be more convenient to migrate first. 
%Our novel approach, named \approach{}, assists developers during the migration process by recommending a set of candidate Java files that could be migrated in the current migration step.

%This work is novel: to our knowledge, no previous work has focused on recommendations of language migrations based on previous migrations done by developers.
%This approach could complement other tools used by developers during migrations, for example, the automated Java-to-Kotlin file converter tool provided by IDEs such as Android Studio.

==> oldtext.tex <==
%\todo{improve or remove}
%Let's give a simple example showed in Figure~\ref{cap6:fig:ranking_evaluation}  that illustrates how  our evaluation works.
%Given as input a project which in its last version (commit \#2) has 4 Java files ($A, C, D$ and $E$), since commit \#2  migrates one file ($A$), it becomes a query that contains one document per file.
%Then, our model generates a ranking of files containing all project files on that version (commit \#2), i.e., a ranking of documents composed of $A$, $C$, $D$ and $E$.
%This ranking is then analyzed based on the position of the \emph{relevant} documents (i.e., those from migrated files such as $A$) to compute the recommendation performance. 


%\todo{????}

%%%%%%% OLD intro



%% Kotlin + Announced
In 2017, Google promoted Kotlin, a programming language that combines functional and object-oriented features, as an official Android language.
More recently, in 2019, Google declared that Android became `Kotlin-first', which means that new API, libraries, documentation will target Kotlin and eventually Java~\cite{AndroidDevelopers2019}.
Since then, Google has advised developers to create new applications using Kotlin instead of Java~\cite{AndroidDevelopers2020b}.


Kotlin is compiled to Java byte-code, which means that 
it is interoperable with Java, i.e., Kotlin code can invoke code written in Java and vice-versa, both running on the same underlying JVM.
Thanks to this interoperability, developers of Java-based Android applications
can:
\begin{inparaenum}[i)]
\item add new Kotlin code and maintain the existing Java code, and/or
\item migrating some parts of theirs apps written in Java code to Kotlin.
\end{inparaenum}
Recent research has shown that the 19\% of Android applications completely migrated from Java to Koltin were \emph{gradually} migrated~\cite{GoisMateus2019}.


%%%%
Moreover, some popular commercial Android applications also gradually migrated from Java to Kotlin.
For instance, Duolingo, a free science-based language education platform~\cite{duolingo_website}, was migrated completely in 2 years. 
Figure~\ref{cap6:fig:duo} shows the evolution of the amount of Java and Kotlin code from Duolingo.
During that period, Java files were progressively migrated to Kotlin, i.e., a commit migrated a subset of Java files, leaving other files in Java.

The \emph{gradual} migration allows developers  
to:
\begin{inparaenum}[\it a)]
\item migrate a subset of Java files, 
\item exhaustively test the migrated code to verify that the migrated code preserves the expected behavior,
and 
\item commit (and eventually release) a new version of their app before continuing with the migration of other files. 
\end{inparaenum}
As Duolingo's developers report~\cite{duolingo_migration2020}, gradual migration allowed them to apply strict testing, code review and code style of each part of the application that was migrated.

Gradual migration faces several challenges.
This paper focuses on a particularly one:
given a version of the program to migrated (composed by not yet migrate and, eventually, some migrated code), a developer should select a set of files that she/he wants to migrate on that migration step.
This selection could be complex as:
\begin{inparaenum}[\it a)]
\item it could exist several candidate files to migrate, and 
\item the wrong selection of files to be migrated could increase the migration effort due to emerging errors~\cite{AbdelAziz2020MigEnterprise,Nizet2018StoryMigration} or additional modifications on files not affected on the migration step. 
\end{inparaenum}
Unfortunately, existing guidelines on migration give high-level pieces of advice or guidance. For instance, Google only suggests that the migration from Java to Kotlin on Android could start by migrating classes in the following order: class model first, then tests, utility functions, and, finally other classes~\cite{AndroidDevelopers2020a}.
%
However, it does not include any guidance for helping developers to decide, for instance, which subset of model classes could be more convenient to migrate first. 

In this paper, we present a novel approach, named \approach{}, that assists developers during the migration process by recommending a set of candidate Java files that could be migrated in the current migration step.

This work is novel: to our knowledge, no previous work has focused on recommendations of language migrations based on previous migrations done by developers.
This approach could complement other tools used by developers during migrations, for example, the automated Java-to-Kotlin file converter tool provided by IDEs such as Android Studio.


We build our approach applying the supervised machine learning technique \emph{learning-to-rank} to create a model that suggests the files to migrates.
The model is learned from real migrations from Java to Kotlin written by developers in open-source projects.
Our intuition is that using information from these migrations, our model captures the rationale behind these migrations.
We trained and evaluated our approach with commits that migrated Java code to Kotlin from \numprint{1457} open-source applications.
To the best of our knowledge, no work has proposed a machine learning-based approach in the context of Android application migration.


%\todo{R2: will there be a general standard, logic, or strategy of how should the migration implement? And how should it be? These should be the questions to be answered or studied first?}

%The result of this paper is: our approach outperforms the random approach by at least 38\%, considering the Mean Average Precision (MAP).\todo{update}
The results of this paper show that \approach{} obtains a mean average precision (MAP metric~\cite{baeza1999modern}) higher than a strategy that follows Google's guideline \cite{AndroidDevelopers2020a}.
We consider that the proposed approach is an initial step towards a fully automated recommendation system to support applications' migration.


The contributions of this paper are:
\begin{itemize}
    \item A benchmark of projects that performed migrations from Java to Kotlin.
    \item An approach that recommends migrations at file level from one programming language to another.
%    \item A static analyzer tool that identifies 12 metrics exclusive to Android applications.\footnote{https://anonymous.4open.science/r/fe5cf980-060b-49ad-81b5-28de22f26360/}\todo{Is this important?? }
\end{itemize}

The paper continues as follows.
Section \ref{sec:term} explains the terminology used along the paper.
Section \ref{sec:approach} characterizes our approach.
Section \ref{sec:methodology} outlines the methodology used to evaluate our approach.
Section \ref{sec:evaluation} reports the evaluation results.
Section \ref{cap6:sec:discussion} discusses the consequences of our results and future work.
Section \ref{sec:threatsvalidity} presents the threats to validity.
Section \ref{sec:relatedwork} presents the related work.
Section \ref{sec:conclusion} concludes the paper.
All the data presented in this paper is publicly available in our appendix: \url{https://anonymous.4open.science/r/fe5cf980-060b-49ad-81b5-28de22f26360}.


\begin{figure}[t]
    \centering
    \includegraphics[width=0.75\columnwidth]{duolingo_evolotion.png}
    \caption{Evolution of the number of lines (LOC, axis X) of Java and Kotlin along with the Duolingo application's migration process~\cite{duolingo_migration2020} since 2014 (Axis Y).}
    %Axis Y shows the amount of code (SLOC) written, and axis X the time from 2014.}
    \label{cap6:fig:duo}
\end{figure}  


%%%%%%%%% OLd Overview


\subsection{Overview}

\todo{for the moment, let's keep this overview here, it's quite specific to move to the new vision section.}

%Our intention is to capture real migrations  
We build our approach \approach{} using information from projects that have done file migrations from one programming language to another.
\todo{move to the concepts section}
Our intuition is that by analyzing those migrations, we can create a model that captures the rationale behind these migrations, i.e., the developers' experience on migrations.
Then we can use it to recommend files to be migrated.


Our approach consists of two phases as Figure~\ref{fig:app:overview} illustrates: 
\begin{inparaenum}[\it a)]
\item the development phase, and 
\item the serving phase. 
\end{inparaenum}
In the development phase, our approach learns a model from migrations from language $lang_1$ (e.g., Java) to $lang_2$ (e.g., Kotlin), done by developers on open-source projects.  
Then, in the serving phase, given a project $P$ as input, the model generated in the development phase is used to recommend file-level migrations: the model produces a list of candidate files to be migrated.
Now, we give a summary of both phases from our approach.

\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.85\textwidth]{methodology.png}
    \caption{We apply two phases: \emph{development}, where we learn a ranking model, and \emph{serving} phase, where we use the model in production.}
    \label{fig:app:overview}
\end{figure*} 

\subsubsection{Development phase}
\label{cap6:sec:design:approach:dev}


\approach{} is built using learning to rank, a supervised machine learning algorithm. Consequently, we need to provide example data to train our model.
Each example is described by a \emph{vector} of measurements or \emph{features} and a label that denotes the category or class the example belongs to~\cite{Hall1998}.
In our case, we use data from projects that have been migrated from one programming language to another to create \approach{}'s training set.
To this end, for each commit of these projects, we analyze their files to create a \emph{vector} of features that describe them by extracting a set of metrics and classifying them as migrated or not migrated (label).
These vectors are the training data used by our approach to learning a model.
Finally, once we trained our model, it is deployed, and it is ready to be used in the serving phase.


\subsubsection{Serving phase}
\label{sec:serving}

In the serving phase, our approach takes as input a program $P$, written partially or totally using $lang_1$, which developers aim to migrate to $lang_2$. 
As done in the development phase, our approach extracts features from the project's files, i.e., candidates files to migrate, and creates for each file one vector of features, as done during the development phase.
These vectors are given as input to our model.
Finally, using this information, the model learned in the development phase sorts the project's files according to their relevance and returns the list of recommended files to be migrated.


%Figure~\ref{cap6:fig:ranking_overview} shows an example of this phase. 
Let us show an simple example for describing this phase.
The approach takes as input a project composed of 5 files where 4 files ($A.lang_1$, $B.lang_1$, $C.lang_1$ and $E.lang_1$) could be migrated, and one $D.lang_2$ already migrated.
The learned rank model ranks the 4 files based on the experience of developers by migrating similar files (i.e., similar vector features). 
In this example, the developer could start migrating the files at the top of the recommendation, e.g., $E.lang_1$, then testing the migrated app, committing the changes, and generating a new version to publish. 
Those activities conform one step on the gradual migration process.
Note that in migrations that involve fully interoperable languages (e.g., Java and Kotlin) the migrated files (e.g., $D.lang_2$) could continue interacting with the not migrated (e.g., $B.lang_1$).

%To our knowledge, all existing guidelines on migration give high-level pieces of advice or guidance. 
%For instance, Google only suggests that the migration from Java to Kotlin on Android could start by migrating classes in the following order: class model first, then tests, utility functions, and, finally other classes~\cite{AndroidDevelopers2020a}.
%However, it does not include any guidance for helping developers to decide, for instance, which subset of model classes could be more convenient to migrate first. 
%Our novel approach, named \approach{}, assists developers during the migration process by recommending a set of candidate Java files that could be migrated in the current migration step.

%This work is novel: to our knowledge, no previous work has focused on recommendations of language migrations based on previous migrations done by developers.
%This approach could complement other tools used by developers during migrations, for example, the automated Java-to-Kotlin file converter tool provided by IDEs such as Android Studio.
